Analyzing Font Style Usage and Contextual Factors in Real Images

There are various font styles in the world. Different styles give different impressions and readability. This paper analyzes the relationship between font styles and contextual factors that might affect font style selection with large-scale datasets. For example, we will analyze the relationship between font style and its surrounding object (such as ``bus'') by using about 800,000 words in the Open Images dataset. We also use a book cover dataset to analyze the relationship between font styles with book genres. Moreover, the meaning of the word is assumed as another contextual factor. For these numeric analyses, we utilize our own font-style feature extraction model and word2vec. As a result of co-occurrence-based relationship analysis, we found several instances of specific font styles being used for specific contextual factors.

==> ArchivedComments <==
【Adobe VFR realの説明】
%synthgerの合成画像を用いて学習したResNet18ベースのモデルの評価をとして、実画像のラベル付きのデータセットであるAdobe Visual Font Recognition (VFR)を使用
% https://paperswithcode.com/dataset/adobevfr-real
%4,384 real-world test images with reliable labels, 617 classes
%アスペクト比を保ったまま高さを64に。幅が128より小さいときは幅が128以上になるまで同じ画像を連結する.モデルの入力が64,128のため。
%これはadobeのフォントラベルが付与されているので、モデルの学習したgoogle fontでのfont classifierでの性能評価はできない。他の手法を使用。


【Open images v4の説明】
%竹下さんから頂いたデータセットを使用。
%Open imgには、オブジェクトのBboxデータはないので、竹下さんが以前の研究で抽出したBboxのデータを使用。
%竹下さんの論文の内容そのまま（OpenImages v4の説明）
%We used the training image set of OpenImages v4 as a dataset to analyze the object-word co-occurrence. Among 1,910,098 images in the dataset, 1,743,042 images with the bounding boxes of 600 predefined object classes are used; that is, the images with no object bounding box are discarded. The dataset contains 14,610,229 object bounding boxes in total; that is, on average, each image contains about eight object bounding boxes

【Book cover dataetのタイトル領域検出】
%207,572枚の書籍表紙画像を用い，そのタイトル部の文字領域をフォントスタイル情報の傾向の分析に使用した．書籍表紙中の文字領域の抽出にはCRAFTを使用し，その文字領域に対し文字認識を行った.なお，抽出した文字領域の高さが15pixel以下の単語は除外した．文字認識には文献で最も認識精度の高かったモデルTPS-ResNet-BiLSTM-Attnを使用した．その文字認識結果と書籍表紙のメタデータに含まれるタイトル情報を照合し，タイトルに相当する部分のみの単語を選出した．その後，stop words，固有名詞，数字，複合語，及び出現回数が10回未満の単語は除外した．また，lemmatizer(nltk)を使用して時制など単語の表記を統一した．結果的に，書籍表紙画像からは，8,384種類の単語が語彙として得られた．ただし，後述のフォントスタイル情報を用いた単語分散表現の獲得では，Google News corpusを用いて単語分散表現が事前学習済みのWord2Vecを使用するために，その学習時に用いられていない単語（特殊な固有名詞や造語等）は対象にできない．よって，本実験を通して使用する単語は，Google News corpusによる300万単語と書籍表紙タイトル部の単語の積集合を取り，7,883単語となった．


【スタイル特徴抽出CNNについて】
%ResNet18をベースとして、最終層を変更したもの。200次元のフォント特徴を得るためのfcと200フォント分類のためのfc
%モデルの汎化性向上のdropoutの付加
%【元の手法】conv -> ave pool -> fc(200dim)
%【提案手法】conv -> ave pool -> fc(200dim) -> relu -> dropout(0.25) -> fc(200dim)
%パラメータ
%optimizer = adam,
%learning rate = 0.001,
%batch size = 64
%この条件で、synthtigerで作った200,000の画像のデータセットで学習。
%また、汎化性能を上げるため？アルファベットの列のみでフォントを判別しないように、毎エポックごと、64,128+の入力画像において、64,128でランダムで切り抜きを行いました。%たとえば、[64,130]の画像だと入力は[64,:128],[64,1:129],[64,2:130]がランダムって感じです。
%synthtigerで生成した200fontの合成画像各1,000枚ずつの合計200,000画像を使用。
%200フォントはgoogle fontのfont familyのserif,sans seif, handwriting, displayから選択
%200font(serif:40, sans-serif:40, handwriting:40, display:80)
%各font familyの中で、同じようなフォントが含まれないように、(△-regular,△-bold)や(■◇-regular,■◯-regular,■★-italic)などが含まれないようにし、ランダムに選択。
%synthtigerには、文字を傾けたりするような変化も含まれているので、それをなくしました。italic出ないフォントもitalicのようになったりするため。
%画像の幅＞高さの画像を各フォントあたり1000画像生成
%アスペクト比を保ったまま高さを64に。幅が128より小さいときは幅が128以上になるまで同じ画像を連結する。モデルの入力が64,128のため。
%サイズが小さいが画像をゼロパディングではなく、同じ画像を連結するのは、ゼロパディングをすると、パディングが可視化した際に集まっていたので。
%文字列はmjsynthのコーパスを使用。synthtigerにもともと入っていたもの.MJsynthという合成画像生成の手法があるようです


【AdobeVFR real解析】
\begin{tabular}{lll}
\hline
\# clusters & Adjusted mutual information & Completeness score\\
\hline
64 & 0.2645 & 0.5962\\
614 & 0.1590 & 0.6204\\
\hline
\end{tabular}
%評価指標では、クラスタリングの結果を用いるので、64と614(617fontとAdobe VFRにはあったが、画像データのないものがあったので、それを引いた数)でクラスタリングして性能を評価。
% 2つの評価指標
% ①adjusted mutual info
% 64クラスタのとき
% 0.2645300645311352
% 614クラスタのとき
% 0.15896479156120458

% ②completeness score
% 64クラスタのとき
% 0.5962279456691426
% 614クラスタのとき
% 0.6203700341817922

%また、sysnthtigerを用いて学習したフォント特徴抽出器にVFRデータセットの画像を入力して特徴を抽出
%その特徴をtsneで2次元に次元削減を行った。
%全データの表示は見にくいので、ランダムに10フォントの画像を選択しtsneで可視化しました。
%VFRのデータセットはフォントごとのデータ数にかなり偏りがあり、数データしかないものも有るため、クラスタリング結果が良くないように見える気がしてます。
% ==============================================
\begin{figure}[t]
\centering
\includegraphics[keepaspectratio,scale=0.3]{images/tsne_points_VFR_random.pdf}
\caption{Visualization of the style features of the Adobe VFR dataset based on $t$-SNE}  \label{fig:tsne_VFR} 
\end{figure}
% ==============================================

% ==============================================
\begin{table}[t]
\caption{Evaluation measures for clustering results of the extracted style features on the AdobeVFR read dataset}
\begin{tabular}{ll}
\hline
\# clusters & Adjusted mutual information\\
\hline
64 & 0.2645 \\
614 & 0.1590 \\
\hline
\end{tabular}
\label{table:AMI}
\end{table}
% ==============================================

【book cover解析結果】
% ==============================================\
%------------------------------------------------------------
%データの基礎知識
%--------------------wordの頻出カウント(in BNC)--------------------
%単語の種類の合計　5027 ←BNCに含まれているもに絞っています。絞らないとtop3にアルファベット一文字とか入ったりするので。
%BNCに含まれるものに制限しているので、竹下さんのように、topN単語をBNCでの頻出ランキングに変換も可能
%nltkでstop wordを除き、w2vで使用可能であり、BNCの頻出単語であるもの。

%BNC(british national corpus）の引用先　「竹下さんと同様」
%http://www.kilgarriff.co.uk/bnc-readme.html
% Top 40 にしました。後で40個使うので。！！
%頻出単語トップNの算出（今回はtop40).順番は図の通り。　とりあえず入れたので、後で図を変更して差し替えOKです。
%後でtop40に入れ換えれるなら入れ替える。
\begin{figure}[t]
 \centering
 \includegraphics[keepaspectratio, scale=0.5]{images/word_count_v4.pdf}
\caption{Top 40 frequent words in Open Images Dataset. Words are displayed only if they are included in the British national corpus (BNC).}  \label{fig:OpenImg_top40word_in_BNC}
\end{figure}
% ==============================================
%--------------------objectの頻出カウント--------------------
%頻出オブジェクトトップNを算出（今回は30）
%オブジェクトの種類の合計　578
Fig.~\ref{fig:OpenImg_top30object} shows the top 30 frequent objects in the Open Image dataset. The total number of detected object types was 578.
% ==============================================
%頻出オブジェクトトップ30の算出、順番は図の通り。
\begin{figure}[t]
 \centering
  \includegraphics[keepaspectratio, scale=0.5]{images/object_count_v4.pdf}
\caption{Top 30 frequent objects in Open Images}  \label{fig:OpenImg_top30object}
\end{figure}
% ==============================================
